Compressive Sampling Approach for Image Acquisition with Lensless Endoscope

The lensless endoscope is a promising device designed to image tissues in vivo at the cellular scale. The traditional acquisition setup consists in raster scanning during which the focused light beam from the optical fiber illuminates sequentially each pixel of the field of view (FOV). The calibration step to focus the beam and the sampling scheme both take time. In this preliminary work, we propose a scanning method based on compressive sampling theory. The method does not rely on a focused beam but rather on the random illumination patterns generated by the single-mode fibers. Experiments are performed on synthetic data for different compression rates (from 10 to 100% of the FOV).

==> pics/fig_SNR-vs-compression_centered-samples.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			font = \small,
			grid = major,
			grid style = {dotted},
			height = 5.5cm,
			width = \linewidth,
			axis lines = left,
			xmin = 0.09,
			%ymax = 20.5, ymin = 0,
			ylabel = {SNR $\left[\text{dB}\right]$},
	    	xlabel = {Ratio $M/N$},
			legend cell align = {left},
    		legend style = {at = {(1.02,0.02)}, font = \footnotesize,
      		anchor = south east,column sep = 0.1cm, draw = none, fill = none},
      		cycle list name=black white,
      		legend entries={Focused PSF after calibration,PSF from $P$ random patterns,Standard deviation}
			]
			
			\addlegendimage{no marks,black,dashed}
			\addlegendimage{no marks,black,solid}	
			\addlegendimage{no marks,gray!50,very thick,solid}	

			% Data importation	
			% ----------------							 	 
			\pgfplotstableread{data/NBDx_Tissue_CS_centered-samples_focusedKernel-M1_GaussianNoise-BSNR40_xPrior-TV_ADMM_20Trials.dat}\dataFocusMOne
			\pgfplotstableread{data/NBDx_Tissue_CS_centered-samples_speckleKernel-M1_GaussianNoise-BSNR40_xPrior-TV_ADMM_20Trials.dat}\dataSpeckleMOne
			\pgfplotstableread{data/NBDx_Tissue_CS_centered-samples_speckleKernel-M2_GaussianNoise-BSNR40_xPrior-TV_ADMM_20Trials.dat}\dataSpeckleMTwo
			\pgfplotstableread{data/NBDx_Tissue_CS_centered-samples_speckleKernel-M4_GaussianNoise-BSNR40_xPrior-TV_ADMM_20Trials.dat}\dataSpeckleMFour

			% Focused/Calibrated PSF
			% ----------------------
			% Standard deviation
%			\addplot+ [name path = A, no marks, forget plot,gray] table[x expr = 100*\thisrowno{0}, y expr = \thisrowno{1}+\thisrowno{2}, y index = 0] {\dataFocusMOne};
%			\addplot+ [name path = B, no marks, forget plot,gray] table[x expr = 100*\thisrowno{0}, y expr = \thisrowno{1}-\thisrowno{2}, y index = 0] {\dataFocusMOne};
%			\addplot+ [opacity = 0.5, forget plot, fill = gray!50] fill between [of = A and B];
			
			% Mean
			\addplot+ [dashed, mark=*, mark size=1pt, mark options={color=black,solid}] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}, y index = 0] {\dataFocusMOne};
			
			
			% Random pattern (M=1)
			% --------------------
			% Standard deviation
			\addplot+ [name path = A, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}+\thisrowno{2}, y index = 0] {\dataSpeckleMOne};
			\addplot+ [name path = B, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}-\thisrowno{2}, y index = 0] {\dataSpeckleMOne};
			\addplot+ [opacity = 0.5, forget plot,fill = gray!50] fill between [of = A and B];
			
			% Mean
			\addplot+ [black, solid, mark=*, mark size=1pt, mark options={color=black,solid}] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}, y index = 0] {\dataSpeckleMOne} node[font=\footnotesize,rotate=25, anchor=south,pos=0.72,yshift=0.5ex] {$P=1$};
			
			
			% Random pattern (M=2)
			% --------------------
			% Standard deviation
			\addplot+ [name path = A, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}+\thisrowno{2}, y index = 0] {\dataSpeckleMTwo};
			\addplot+ [name path = B, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}-\thisrowno{2}, y index = 0] {\dataSpeckleMTwo};
			\addplot+ [opacity = 0.5, forget plot,fill = gray!50] fill between [of = A and B];
			
			% Mean
			\addplot+ [black,solid, mark=*, mark size=1pt, mark options={color=black,solid}] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}, y index = 0] {\dataSpeckleMTwo} node[font=\footnotesize,rotate=44, anchor=south,pos=0.66,yshift=0.5ex] {$P=2$};
			
			
			% Random pattern (M=4)
			% --------------------
			% Standard deviation
			\addplot+ [name path = A, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}+\thisrowno{2}, y index = 0] {\dataSpeckleMFour};
			\addplot+ [name path = B, no marks, forget plot,draw=none,gray] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}-\thisrowno{2}, y index = 0] {\dataSpeckleMFour};
			\addplot+ [opacity = 0.5, forget plot,fill = gray!50] fill between [of = A and B];
			
			% Mean
			\addplot+ [black,solid,mark = *, mark size=1pt, mark options={color=black,solid}] table[x expr = \thisrowno{0}, y expr = \thisrowno{1}, y index = 0] {\dataSpeckleMFour} node[font=\footnotesize,rotate=13, anchor=south,pos=0.9,yshift=0.3ex] {$P=4$};
			
			
			%\legend{Calibrated PSF, Random pattern PSF ($M=1$), Random pattern PSF ($M=2$), Random pattern PSF ($M=4$)}	
			
			
		
		\end{axis} 
	\end{tikzpicture}
	\vskip-1ex
	\caption{Mean SNR (over 20 trials) of restored $128\times 128$ tissue image \emph{versus} $M/N$, \emph{i.e.}, the ratio between the number of observations and the number of pixels in the FOV. The BSNR of observations is 40\,dB.}
	\label{fig:SNR-vs-compression_centered-samples}
	\vskip-2ex
\end{figure}
